Multi-field Visualization: Trait design and trait-induced merge trees

Feature level sets (FLS) have shown significant potential in the analysis of multi-field data by using traits defined in attribute space to specify features in the domain. In this work, we address key challenges in the practical use of FLS: trait design and feature selection for rendering. To simplify trait design, we propose a Cartesian decomposition of traits into simpler components, making the process more intuitive and computationally efficient. Additionally, we utilize dictionary learning results to automatically suggest point traits. To enhance feature selection, we introduce trait-induced merge trees (TIMTs), a generalization of merge trees for feature level sets, aimed at topologically analyzing tensor fields or general multi-variate data. The leaves in the TIMT represent areas in the input data that are closest to the defined trait, thereby most closely resembling the defined feature. This merge tree provides a hierarchy of features, enabling the querying of the most relevant and persistent features. Our method includes various query techniques for the tree, allowing the highlighting of different aspects. We demonstrate the cross-application capabilities of this approach through five case studies from different domains.

==> sections/discussion.tex <==
In this paper, we propose methods to enhance the application of Feature level sets (FLS), including support for trait design and the introduction of the trait-induced merge tree (TIMT) to help in the feature selection.
The concept of TIMTs is straightforward compared to previously proposed methods for topological analysis of multi-fields. The computation of feature level sets is simple, and merge tree computation is well-researched and available through open-source libraries. Thus, TIMTs offer a novel approach to topological data analysis for multivariate data and tensor fields, providing valuable insights into the data. This concept allows for the generalization of fundamental topological concepts, as demonstrated with the merge tree. Notions like persistence can be naturally extended to multi-fields or tensor fields, supporting multi-scale analysis.
TIMT-based features simplify feature selection by providing intuitive segmentation of the domain. The user interface supports browsing the segmentation via a legend or slice. However, determining parameters such as persistence thresholds or crown height can be challenging without visual aids. To address this, we plan to equip the framework with a persistence diagram or a tree representation with a cutoff slider, potentially improving the method's usability.
For domain experts or educated users, defining the trait should be straightforward enough to experiment with different notions of traits and features. The introduction of Cartesian traits simplifies the assembly of complex traits and the efficient computation of the necessary distance fields. However, this still requires significant domain knowledge. More automatic methods could be helpful here. The suggestion of point traits using dictionary learning shows potential, but these dictionaries are not yet well understood, and results must be critically evaluated. A remaining crucial decision is determining which attributes to include in the attribute space $\Aspace$. Similarly, specifying an appropriate metric in this space for attributes with different scales and units is not trivial.
From a computational perspective, interpolation artifacts may arise for non-linear derived attributes such as eigenvalues for tensor fields. To compute exact level sets, the data would need to be interpolated in the spatial domain during the ray-marching process instead of pre-computing the distance field. Similar problems might appear in the computation of the merge tree. For a thorough discussion of these aspects of FLS, we refer the reader to \cite{JankowaiHotz2019}.
The FLS implementation used in this article is GPU-based and performed at interactive frame rates for all data sets used. The computation of the merge tree depends on the complexity of the distance field. In our examples, it took less than a minute. Feature extraction based on the methods presented in~\sref{sec:query_methods}   took a comparable amount of time. Additionally, the process of feature extraction can be offloaded to the GPU and should perform at interactive frame rates.in workflows for domain experts.

